Scaling Limit Theorems for Multivariate Hawkes Processes and Stochastic Volterra Equations with Measure Kernel

This paper is devoted to establishing the full scaling limit theorems for multivariate Hawkes processes. Under some mild conditions on the exciting kernels, we develop a new way to prove that after a suitable time-spatial scaling, the asymptotically critical multivariate Hawkes processes converge weakly to the unique solution of a multidimensional stochastic Volterra equation with convolution kernel being the potential measure associated to a matrix-valued extended Bernstein function. Also, based on the observation of their affine property and generalized branching property, we provide an exponential-affine representation of the Fourier-Laplace functional of scaling limits in terms of the unique solutions of multidimensional Riccati-Volterra equations with measure kernel. The regularity of limit processes and their alternate representations are also investigated by using the potential theory of L\'evy subordinators.

==> ElementaryProp.tex <==
 \section{Fourier-Laplace functional of Hawkes processes} \label{Sec.ElementaryProp}
  \setcounter{equation}{0}
 
 In this section, we prove the exponential-affine representation of Fourier-Laplace functional of $(\boldsymbol{N},\boldsymbol{\Lambda})$ given in Theorem~\ref{Thm.FourierLaplaceHP} by following an argument similar to that in \cite[Section~3]{HorstXu2023}.  
 
 A  pair $(\boldsymbol{\tilde{V}},T_\infty)$ with $T_\infty\in (0,\infty]$ and $\boldsymbol{\tilde{V}}\in L^\infty_{\rm loc}([0,T_\infty),\mathbb{C}^d)$ is called a \textit{non-continuable solution} of (\ref{VolRiccati}) if $\boldsymbol{\tilde{V}}$
 satisfies (\ref{VolRiccati}) on $[0,T_\infty)$ and $\|\boldsymbol{\tilde{V}}\|_{L^\infty_{T_\infty}}=\infty$ if $T_\infty<\infty$; we say that $\boldsymbol{\tilde{V}}$ is a {\it global solution} if $T_\infty=\infty$.  
 The existence of a unique non-continuable solution $(\boldsymbol{\tilde{V}},T_\infty)\in L^\infty_{\rm loc}([0,T_\infty);\mathbb{C}^d)\times(0,\infty]$ of (\ref{VolRiccati}) can be obtained by using Banach's fixed point theorem; see e.g.  \cite[p.341-343]{GripenbergLondenStaffans1990}, 
 \beqnn
 \boldsymbol{\tilde{V}} =  \big( \boldsymbol{\tilde{W}} +\boldsymbol{\tilde{V}} \big) * \boldsymbol{\phi}, \quad \mbox{$L(dt)$-a.s.}
 \quad \mbox{with}\quad 
 \boldsymbol{\tilde{W}} :=\boldsymbol{f}+\boldsymbol{g} + \mathcal{W}(\boldsymbol{\tilde{V}}+\boldsymbol{g}+ \boldsymbol{h}) .
 \eeqnn
 Let $ \boldsymbol{V}=\big(  \boldsymbol{\tilde{W}} +\boldsymbol{\tilde{V}} \big) * \boldsymbol{\phi}$ and $\boldsymbol{W} = \boldsymbol{f}+\boldsymbol{g} +\mathcal{W}(\boldsymbol{V}+\boldsymbol{g}+ \boldsymbol{h})$.
 Notice that $\boldsymbol{V} \in  C([0,T_\infty);\mathbb{C}^d)$ and satisfies (\ref{VolRiccati}) for any $t\in[0,T_\infty)$, thus  $(\boldsymbol{V},T_\infty)\in C([0,T_\infty);\mathbb{C}^d)\times(0,\infty]$ of (\ref{VolRiccati}) is the unique non-continuable solution of (\ref{VolRiccati}).
 We establish the existence of a unique global solution in the sequel of this section.
 
  
 
 \begin{proposition}\label{Lemma.FourLapGHP}
 	For row vector functions $\boldsymbol{f},\boldsymbol{g}\in L^\infty_{\rm loc}(\mathbb{R}_+;\mathbb{C}_-^d) $ and $\boldsymbol{h}\in L^\infty_{\rm loc}(\mathbb{R}_+;\mathtt{i}\mathbb{R}^d)$, if $(\boldsymbol{V},T_\infty)\in C([0,T_\infty);\mathbb{C}^d)\times(0,\infty]$ is a  non-continuable solution of (\ref{VolRiccati}), then (\ref{FourLapFunHP}) holds for any $T\in[0,T_\infty)$. 
 
 \end{proposition}
 \proof 
 Recall the function $\boldsymbol{W}$ defined in (\ref{VolRiccati}).   
 For each $T\in[0,T_\infty)$, let 
 \beqnn
 Y_T:=  \boldsymbol{W} *\boldsymbol{\Lambda} (T).
 \eeqnn 
 Taking expectations on both sides of (\ref{SVR}), we see that
 \beqnn
 \mathbf{E} \big[\boldsymbol{\varLambda}(t) \big]=\boldsymbol{H}(t)
 \quad \mbox{and}\quad
 \mathbf{E}\big[Y_T\big]=  \boldsymbol{W} * \boldsymbol{H}  (T).
 \eeqnn 
 We introduce the Doob martingale 
 \beqnn
 Y_T(t):=\mathbf{E}\big[Y_T \big| \mathscr{F}_t\big],\quad t\in[0,T].
 \eeqnn
 By using the martingale representation of the intensity process $\boldsymbol{\varLambda}$ established in Lemma \ref{Lemma.MartRep} along with the stochastic Fubini theorem and the fact that 
 $\boldsymbol{V}=  \boldsymbol{W} *\boldsymbol{R} $,
 \beqlb\label{eqn.3.03}
 Y_T(t)
 = \mathbf{E}[Y_T] + \int_0^T \boldsymbol{W} (T-r) \int_0^{t\wedge r}  \boldsymbol{R}(r-s)d\widetilde{\boldsymbol{N}}(s)dr
 = \mathbf{E}[Y_T] + \int_0^t \boldsymbol{V}(T-s) d\widetilde{\boldsymbol{N}}(s).
 \eeqlb
 Next, we introduce a semimartingale $ \{Z_T(t):t\in[0,T]\}$ by
 \beqlb\label{eqn.3002}
 Z_T(t)
 \ar:=\ar Y_T(t) - \int_0^t \big(\boldsymbol{W}-\boldsymbol{f}+\boldsymbol{h}\big)(T-s) \boldsymbol{\varLambda}(s)ds + \int_0^t  (\boldsymbol{g}+ \boldsymbol{h})(T-s) d\boldsymbol{N}(s)\cr
 \ar=\ar \mathbf{E}[Y_T]-  \int_0^t  \big(\boldsymbol{W}-\boldsymbol{f}-\boldsymbol{g}\big) (T-s) \boldsymbol{\varLambda}(s)ds + \int_0^t  \big(\boldsymbol{g}+ \boldsymbol{h} +\boldsymbol{V} \big)(T-s) d\widetilde{\boldsymbol{N}}(s).
 \eeqlb
 Applying It\^{o}'s formula to $\exp\{Z_T(t) \}$ and then using the definition of $\boldsymbol{W}$, we obtain that
 \beqlb\label{eqn.3008}
 e^{Z_T(t)}= e^{\mathbf{E}[Y_T]} + \int_0^t e^{Z_T(s-)} \big(e^{\boldsymbol{V}+ \boldsymbol{g}+ \boldsymbol{h} } -\mathbf{1}\big) (T-s)  d\widetilde{\boldsymbol{N}}(s),\quad t\in[0,T] , 
 \eeqlb
 which is a $(\mathscr{F}_t)$-local martingale.  If the local martingale were a true martingale, then the desired result follows from 
 \beqnn
 Z_T(T)=  
 \boldsymbol{f}*\boldsymbol{\varLambda}(T) + \boldsymbol{g}* d\boldsymbol{N}(T) + \boldsymbol{h} * d\widetilde{\boldsymbol{N}}(T)
 \eeqnn 
 by taking expectations on both sides of (\ref{eqn.3008}) with $t=T$. 
 
 It remains to prove that $\{ \exp\{Z_T(t) \}: t\in[0,T]  \}$ is a true $(\mathscr{F}_t)$-martingale. 
 We first define the process
 \beqnn
 U_T(t):=  \int_0^t \big(e^{\boldsymbol{V}+ \boldsymbol{g}+ \boldsymbol{h} } -\mathbf{1}\big) (T-s)  d\widetilde{\boldsymbol{N}}(s), \quad t\geq 0.
 \eeqnn
 In view the local integrability of $\boldsymbol{H}$ and the local boundedness of $(\boldsymbol{V},\boldsymbol{g})$, 
 it follows from the Burkholder-Davis-Gundy inequality that 
 \beqnn
 \sup_{t\in[0,T]}\mathbf{E}\big[|U_T(t)|^2\big]
 \ar\leq\ar \sum_{i=1}^d \sup_{t\in[0,T]} \int_0^t\mathbf{E} \big[\varLambda_i(s)\big] \big| e^{(V_i+g_i+h_i)(T-s)}-1\big|^2 ds \cr 
 \ar\leq\ar  \sum_{i=1}^d \sup_{t\in[0,T]} \big| e^{(V_i+g_i+h_i)(t)}-1\big|^2 \cdot \mathcal{I}_{H_i}(T) <\infty
 \eeqnn
 and hence that $ \{U_T(t):t\in[0,T]\}$ is a locally uniformly square integrable $(\mathscr{F}_t)$-martingale. Let
 \beqnn
 \mathcal{E}_{U_T}:= \{\mathcal{E}_{U_T}(t): t\geq 0 \} 
 \eeqnn
 be the Dol\'ean-Dade exponential of $U_T$. By It\^o's formula,
 \beqnn
 \mathcal{E}_{U_T}(t)
 =\exp\Big\{ -\int_0^t  \big(\boldsymbol{W}-\boldsymbol{f}-\boldsymbol{g}\big)(T-s)\boldsymbol{\Lambda}(s) ds + \int_0^t  (\boldsymbol{V}+\boldsymbol{g}+\boldsymbol{h})(T-s) d\widetilde{\boldsymbol{N}}(s)  \Big\}, \quad t\geq 0.
 \eeqnn
 From this and (\ref{eqn.3002}), we see that  
 $ e^{Z_T(t)}=e^{\mathbf{E}[Y_T]}  \mathcal{E}_{U_T}(t) $ for  $t\in[0,T]$.
 Since $ \mathcal{E}_{U_T}$ is a non-negative local martingale it is a super-martingale and so $\mathbf{E}[\mathcal{E}_{U_T}(t)] \leq 1$. It hence suffices to prove that 
 \beqnn
 \mathbf{E}[\mathcal{E}_{U_T}(t)]=1, \quad t\geq 0.
 \eeqnn
 
 To this end, we introduce, for each $t_0\geq 0$ and $n\geq 1$ the quantities
 \beqnn
 \tau_n:=\inf\Big\{ s\geq 0: \max_{i\in\mathtt{D}}\mathcal{I}_{\Lambda_i}(s)\geq n \Big\} \wedge t_0
 \quad\mbox{and}\quad
 \mathcal{E}_{U_T}^{(n)}(t):=  \mathcal{E}_{U_T}(\tau_n \wedge t), 
 \quad t\geq 0. 
 \eeqnn  
 Since  $(\boldsymbol{V},\boldsymbol{g})$ is locally bounded, there exists a constant $C>0$ such that uniformly in $t \in [0,T]$ and $i\in\mathtt{D}$ the following holds:
 \beqnn
 \int_0^t \mathbf{1}_{\{s\leq \tau_n\}}  \varLambda_i (s) \bigg| 1-\big( 1-(V_i+g_i+h_i)(T-s) \big)      e^{(V_i+g_i+h_i)(T-s) }  \bigg|  ds 
 \leq C\cdot \int_0^{\tau_n}\varLambda_i(s) ds \leq C\cdot n. 
 \eeqnn
 Hence, the process $\mathcal{E}_{U_T}^{(n)}$ is a martingale for each $n\geq 1$, due to Theorem~IV.3 in \cite{LepingleMemin1978}. 
 Thus, 
 \beqnn 
  1 = \mathbf{E}\big[\mathcal{E}_{U_T}^{(n)}(t_0)\big]
  \ar=\ar \mathbf{E}\big[\mathcal{E}_{U_T}^{(n)}(t_0); \tau_n = t_0\big] + \mathbf{E}\big[\mathcal{E}_{U_T}^{(n)}(t_0);\tau_n<t_0\big]  \\
  \ar=\ar \mathbf{E}\big[\mathcal{E}_{U_T}(t_0);\tau_n= t_0\big] + \mathbf{E}\big[\mathcal{E}_{U_T}^{(n)}(\tau_n);\tau_n<t_0\big] . 
 \eeqnn
 By the monotone convergence theorem and the fact that $\tau_n \to t_0$ a.s.~as $n\to\infty$, 
 \beqnn
  \mathbf{E}\big[\mathcal{E}_{U_T}(t_0); \tau_n=t_0 \big]\to  \mathbf{E}\big[ \mathcal{E}_{U_T}(t_0) \big]
 \eeqnn
 and so it suffices to prove that $\mathbf{E}[\mathcal{E}_{U_T}^{(n)}(\tau_n);\tau_n<t_0] \to 0$ as $n\to\infty$. 
 
 To this end, we define a probability law  $\mathbf{Q}_T^{(n)}$ on $(\Omega,\mathscr{F},\mathscr{F}_t)$ by 
 \beqnn
 \frac{d  \mathbf{Q}_T^{(n)} }{ d \mathbf{P} } = \mathcal{E}_{U_T}^{(n)} (\tau_n). 
 \eeqnn
 By the definition of $\tau_n$ and Chebyshev's inequality it follows that
 \beqnn
 \mathbf{E}\big[\mathcal{E}_{U_T}^{(n)}(\tau_n); \tau_n<t_0 \big]  =\mathbf{Q}_T^{(n)} \big(\tau_n<t_0 \big) = \mathbf{Q}_T^{(n)} \Big( \max_{i\in\mathtt{D}}\mathcal{I}_{\varLambda_i} (t_0) \geq n\Big) \leq \frac{1}{n}\sum_{i=1}^d \mathbf{E}^{\mathbf{Q}_T^{(n)}}\big[ \mathcal{I}_{\varLambda_i}(t_0)\big]  
 \eeqnn
 and hence the desired result holds if we can establish a uniform upper bound on $\mathbf{E}^{\mathbf{Q}_T^{(n)}}\big[ \mathcal{I}_{\varLambda_i}(t_0)\big]$. In what follows we prove that there exists $\beta > 0$ such that
 \beqnn
 \sup_{n\geq 1}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t_0) \big] 
 \leq  2 e^{\beta t_0}  \mathcal{I}_{\boldsymbol{H}} (t_0).
 \eeqnn
 
 As  in~\cite[Section~2]{HorstXu2021}, on an extension of the original probability space we can define $d$ independent Poisson random measures (PRMs) $\{N_{0,i}(ds,dz): i\in\mathtt{D}\}$ on $(0,\infty)^2$ with intensity $ds dz$ such that 
 \beqlb
 N_i(t)= \int_0^t \int_0^{\varLambda_i(s-)} N_{0,i}(ds,dz)
 \quad{and} \quad
 \varLambda_i(t) =  H_i (t)+ \sum_{j=1}^d \int_0^t  \int_0^{\varLambda_i(s-)}R_{ij}(t-s)  \widetilde{N}_{0,j}(ds,dz ), \label{eqn.3001}
 \eeqlb
 for any $t\geq0$ and $i\in\mathtt{D}$, where $\widetilde{N}_{0,j}(ds,dz ):= N_{0,j}(ds,dz )-dsdz$ is the compensated random measure.  By Girsanov's theorem for random measures as stated in, e.g.~Theorem~3.17 in \cite[p.170]{JacodShiryaev2003}, the PRM $N_{0,i}(ds,dz)$ is a random point measure under $\mathbf{Q}_T^{(n)}$ with intensity 
 \beqnn
 \mathbf{1}_{\{ s\leq \tau_n \}}\cdot \exp \{ (V_i+g_i+h_i)(T-s) \}  ds dz.
 \eeqnn
 Moreover, the second equation in (\ref{eqn.3001}) - which holds a.s.~under the measure $\mathbf{P}$ - induces the following equality in distribution under the measure $\mathbf{Q}_T^{(n)}$: 
 \beqnn
 \varLambda_i (t)\ar \overset{\rm d}=\ar   H_i (t) + \sum_{j=1}^d \int_0^t  \int_0^{\varLambda_j(s-)}R_{ij}(t-s)  \widetilde{N}_{0,j}(ds,dz ) \cr
 \ar\ar    + \sum_{j=1}^d \int_0^t \mathbf{1}_{\{ s\leq \tau_n \}} R_{ij}(t-s) \varLambda_j (s) \big(e^{(V_j+g_j+h_j)(T-s)}-1 \big)ds , \quad i\in\mathtt{D}, t \geq 0.  
 \eeqnn 
 Taking expectations on both sides of the above equation and then integrating them over $[0,t]$ yields that
 \beqnn
 \int_0^t \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[ \boldsymbol{\varLambda} (s) \big]ds  
 \ar\leq\ar \mathcal{I}_{\boldsymbol{H}}(t) + C_0  \int_0^t dr \int_0^r  \boldsymbol{R}(t-s)   \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \boldsymbol{\varLambda} (s) \big] ds, 
 \eeqnn
 for some constant $C_0>0$ that is independent of $t$ and $n$. 
 Applying Fubini's theorem to the term on the left-hand side of the equality and to the double integral on the right-hand side of the inequality and then using the fact that $ \mathcal{I}_{\Lambda }$ is non-decreasing we see that
 \beqnn
 \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big] 
 \ar\leq\ar   \mathcal{I}_{H_\mu} (t) + C_0 \int_0^t\boldsymbol{R}(t-s)   \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }( s) \big]  ds.  
 \eeqnn  
 From (\ref{Resolvent}),  for any constant $\beta>0$ such that the norm  
 \beqnn
 \sum_{i,j=1}^d\int_0^\infty e^{-\beta t}  \phi_{ij}(t)dt \leq \frac{1/2}{1+C_0},
 \eeqnn
 we have 
 \beqnn
 \sum_{i,j=1}^d \int_0^\infty e^{-\beta t}R_{ij}(t)dt   \leq   \sum_{i,j=1}^d\int_0^\infty e^{-\beta t}  \phi_{ij}(t)dt \Big(1-\sum_{i,j=1}^d\int_0^\infty e^{-\beta t}  \phi_{ij}(t)dt\Big)^{-1} \leq \frac{1}{1+2C_0}.
 \eeqnn 
 and hence 
 \beqnn
 \sup_{t\in[0,t_0]} e^{-\beta t} \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big]  
 \ar\leq\ar \sup_{t\in[0,t_0]} e^{-\beta t} \mathcal{I}_{\boldsymbol{H}} (t) +\sup_{t\in[0,t_0]}  C_0 \int_0^t  e^{-\beta (t-s)} \boldsymbol{R}(t-s) e^{-\beta s}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }( s) \big]  ds\cr 
 \ar\leq\ar \sup_{t\in[0,t_0]} e^{-\beta t} \mathcal{I}_{\boldsymbol{H}} (t) + C_0\cdot    \int_0^\infty e^{-\beta t}\boldsymbol{R}(t)dt   \cdot \sup_{t\in[0,t_0]} e^{-\beta t}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big]\cr
 \ar\leq\ar  \sup_{t\in[0,t_0]} e^{-\beta t} \mathcal{I}_{\boldsymbol{H}} (t) + C_0\cdot    \sum_{i,j=1}^d \int_0^\infty e^{-\beta t}R_{ij}(t)dt \cdot \sup_{t\in[0,t_0]} e^{-\beta t}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big]\cr
 \ar\leq\ar  \mathcal{I}_{\boldsymbol{H}} (t_0) + \frac{1}{2}\cdot  \sup_{t\in[0,t_0]} e^{-\beta t}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big] ,
 \eeqnn
 which yields that $\sup_{n\geq 1} \sup_{t\in[0,t_0]} e^{-\beta t}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big] \leq 2\cdot  \mathcal{I}_{\boldsymbol{H}} (t_0)$.
 Consequently, 
 \beqnn
 \sup_{n\geq 1}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t_0) \big] 
 \leq e^{\beta t_0} \sup_{n\geq 1} \sup_{t\in[0,t_0]} e^{-\beta t}  \mathbf{E}^{\mathbf{Q}^{(n)}_T}\big[  \mathcal{I}_{\boldsymbol{\varLambda} }(t) \big]
 \leq  2 e^{\beta t_0}  \mathcal{I}_{\boldsymbol{H}} (t_0).
 \eeqnn
 \qed
 
 
 \medskip
 \textit{\textbf{Proof of Theorem~\ref{Thm.FourierLaplaceHP}.}} 
 The existence and uniqueness of a non-continuable solution $(\boldsymbol{V},T_\infty)$ follows from standard arguments. 
 In view of Lemma~\ref{Lemma.FourLapGHP} it remains to prove that  $T_\infty=\infty$ and  that $ {\tt Re}\boldsymbol{V} \leq 0$. 
 For each fixed $j\in \mathtt{D}$, let 
 \beqnn
 \boldsymbol{\phi}_{\cdot j}:=(\boldsymbol{\phi}_{i j})_{i\in\mathcal{D}}^{\rm T}
 \quad \mbox{and}\quad 
 \boldsymbol{R}_{\cdot j}:=(\boldsymbol{R}_{i j})_{i\in\mathcal{D}}^{\rm T}
 \eeqnn
 be the $j$-columns of $\boldsymbol{\phi}$ and $\boldsymbol{R}$ respectively. 
 Choosing $\boldsymbol{\mu}=\boldsymbol{\phi}_{\cdot j}$, we see that  for   $ \boldsymbol{f}, \boldsymbol{g}\in L^\infty_{\rm loc}(\mathbb{R}_+;\mathbb{C}_-^d) $  and $\boldsymbol{h}\in L^\infty_{\rm loc}(\mathbb{R}_+;\mathtt{i}\mathbb{R}^d)$, 
 \beqnn
 \boldsymbol{H}= \boldsymbol{\phi}_{\cdot j}+\boldsymbol{R}* \boldsymbol{\phi}_{\cdot j}=\boldsymbol{R}_{\cdot j}
 \quad\mbox{and}\quad
 \boldsymbol{W} * \boldsymbol{H} = \boldsymbol{W} * \boldsymbol{R}_{\cdot j}= V_j.
 \eeqnn
 Taking these back into equation (\ref{FourLapFunHP}) shows that 
 \beqnn
 \mathbf{E}\Big[\exp \big\{  \boldsymbol{f} *  \boldsymbol{\Lambda}(T) +  \boldsymbol{g} * d \boldsymbol{N}(T)+ \boldsymbol{h} * d\widetilde{\boldsymbol{N}}(T) \big\}\Big]
 = e^{  V_j(T) },
 \quad  T\in[0,T_\infty). 
 \eeqnn 
 It hence follows that 
 \beqnn
 \exp\big\{{\tt Re}V_j(T)\big\} = \big|\exp\big\{  V_j(T) \big\}\big|
 \ar\leq\ar \mathbf{E}\Big[\Big|\exp\Big\{  \boldsymbol{f} *  \boldsymbol{\Lambda}(T) +  \boldsymbol{g} * d \boldsymbol{N}(T)+ \boldsymbol{h} * d\widetilde{\boldsymbol{N}}(T) \Big\}\Big|\Big]\cr
 \ar=\ar\mathbf{E}\Big[ \exp\Big\{ {\tt Re}\Big( \boldsymbol{f} *  \boldsymbol{\Lambda}(T) +  \boldsymbol{g} * d \boldsymbol{N}(T)+ \boldsymbol{h} * d\widetilde{\boldsymbol{N}}(T) \Big) \Big\} \Big]\leq 1 , 
 \eeqnn
 and hence that ${\tt Re}V_j(T) \leq 0$. Furthermore, from (\ref{VolRiccati}) we can see that 
 \beqnn
 {\tt Re}(V_j)= {\tt Re}\big((\boldsymbol{f}-\boldsymbol{h} )*\boldsymbol{\phi}_{\cdot j}\big)+ \Big(\exp\{{\tt Re}(V_i+g_i+h_i)\}\cos ({\tt Im}(V_i+g_i+h_i)) -1\Big)_{i\in\mathtt{D}}*\boldsymbol{\phi}_{\cdot j}.
 \eeqnn
 Since ${\tt Re}(V_i+g_i+h_i)={\tt Re}(V_i+g_i)\leq 0$, we have that $ {\tt Re}\big((\boldsymbol{f}-\boldsymbol{h} )*\boldsymbol{\phi}_{\cdot j}\big)={\tt Re}\big(\boldsymbol{f} *\boldsymbol{\phi}_{\cdot j}\big)$ and
 \beqnn
 {\tt Re}\big(\boldsymbol{f} *\boldsymbol{\phi}_{\cdot j}\big)
 \geq {\tt Re}(V_j)\geq
  {\tt Re}\big(\boldsymbol{f} *\boldsymbol{\phi}_{\cdot j}\big) -2\cdot\big(\mathbf{1}*\boldsymbol{\phi}_{\cdot j} \big).
  \eeqnn
 Similarly, we also have 
 \beqnn
 {\tt Im}(V_j) = {\tt Im} \big((\boldsymbol{f}-\boldsymbol{h})*\boldsymbol{\phi}_{\cdot j}\big)+ \Big(\exp\{{\tt Re}(V_i+g_i+h_i)\}\sin \big({\tt Im}(V_i+g_i+h_i)\big) \Big)_{i\in\mathtt{D}}*\boldsymbol{\phi}_{\cdot j},
 \eeqnn
 and $ |{\tt Im}(V_j)| \leq \big|{\tt Im} \big((\boldsymbol{f}-\boldsymbol{h})*\boldsymbol{\phi}_{\cdot j}\big) \big|+\mathbf{1} * \boldsymbol{\phi}_{\cdot j}$.
 These estimates also yield that  $T_\infty=\infty$ and $\boldsymbol{V}\in C(\mathbb{R}_+;\mathbb{C}_-^d)$. 
 \qed 
 

==> ProofMainThm02.tex <==
 
 \section{Proofs of Lemma~\ref{Lemma.201} and Proposition~}
 \label{ProofMainThm02}
 \setcounter{equation}{0}
 
 
 
 
 
 

  

 
 
 
 

 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
